Fine-Grained Fashion Similarity Learning by Attribute-Specific Embedding Network

This paper strives to learn fine-grained fashion similarity. In this similarity paradigm, one should pay more attention to the similarity in terms of a specific design/attribute among fashion items, which has potential values in many fashion related applications such as fashion copyright protection. To this end, we propose an Attribute-Specific Embedding Network (ASEN) to jointly learn multiple attribute-specific embeddings in an end-to-end manner, thus measure the fine-grained similarity in the corresponding space. With two attention modules, i.e., Attribute-aware Spatial Attention and Attribute-aware Channel Attention, ASEN is able to locate the related regions and capture the essential patterns under the guidance of the specified attribute, thus make the learned attribute-specific embeddings better reflect the fine-grained similarity. Extensive experiments on four fashion-related datasets show the effectiveness of ASEN for fine-grained fashion similarity learning and its potential for fashion reranking.

==> sup/Analysis.tex <==
\subsection*{Quantitative Analysis}
    \subsubsection*{Results on DARN}
    Table \ref{tab:DARN} shows the results of our model and CSN\cite{veit2017} on DARN dataset. It is still that our model performance is higher than csn on each attribute, and the final result of our model is 53.37\%, while CSN's is 50.28\% The values here are generally larger than DeepFashion's, and the results are similar to those on FashionAI dataset, because the two datasets are similar, the property values are very specific, and the images of different property values can be well distinguished.
    \subsubsection*{Results on DeepFashion}
    Table \ref{tab:DeepFashion} shows the results of our model and CSN model on DeepFashion dataset. Our model has more or less performance improvement in each attribute, and finally it is close to 1\% overall. The overall value here is small because first of all, DeepFashion itself has 1K+ attribute values. A large number of attribute values bring great difficulty to the network. Secondly, these attribute values are mostly abstract. It's hard to see the difference in the picture between different attribute values, which is the main reason for the low performance.




    \begin{table*}[tb!]
    \centering
    \caption{\textbf{The mean mAP results in DARN dataset}}
    \label{tab:DARN}
    \scalebox{0.7}{
        \begin{tabular}{ccccccccccc}
        \toprule
        Method&clothes category&clothes button&clothes color&clothes length&clothes pattern&clothes shaoe&collat shaoe&sleeve length&sleeve shape&mAP\\
        \midrule
        ConditionalDisNet & 36.69 & 46.96 & 51.35 & 56.47 & 54.49 & 60.02 & 34.18 & 80.11 & 60.04 & 53.31\\
        \midrule
        ConditionalSimNet & 33.65 & 44.09 & 42.50 & 55.11 & 53.06 & 56.89 & 28.85 & 79.15 & 59.22 & 50.15\\
        \bottomrule
        \end{tabular}
    }
    \centering
    \caption{\textbf{The mean mAP results in DeepFashion dataset}}
    \label{tab:DeepFashion}
    \scalebox{1.0}{
        \begin{tabular}{ccccccc}
        \toprule
        Method&texture-related&fabric-related&shape-related&part-related&style-related&mAP\\
        \midrule
        ConditionalDisNet & 15.13 & 7.11 & 12.39 & 5.51 & 3.56 & 8.74\\
        \midrule
        ConditionalSimNet & 13.74 & 6.24 & 11.76 & 4.66 & 3.18 & 7.91\\
        \bottomrule
        \end{tabular}
    }
    \end{table*}

==> sup/DARN.tex <==
\subsection*{Experiment on DARN}
    \subsubsection*{Setup}
    DARN\cite{huang2015DARNdataset} is a dataset consisting of attribute prediction dataset and street2shop retrieval dataset. Since we only search in in-shop cloth, we use DARN's attribute prediction dataset to train our model. DARN attribute prediction dataset contains 253,983 pictures, 9 attributes, and a total of 185 attribute values (including N/A). For the sake of the network, we only got 214,619 images, which are divided in the same way as DeepFashion.
    \subsubsection*{Results}
    As well as DeepFashion and FashionAI, We implement 6 models on DARN dataset.
    Table \ref{tab:DARN} shows the results of these 6 models on DARN dataset.  The values here are generally larger than DeepFashion's, and the results are similar to those on FashionAI dataset, because the two datasets are similar, the property values are very specific, and the images of different property values can be well distinguished.
    It is still that our model performance is higher than csn on each attribute, and the final result of our model is 53.31\%, while CSN's is 50.86\%. The result of ASEN without ASA and without ACA are 51.39\% and 48.02\% respectively.


    \begin{table*} [tb!]
    \renewcommand{\arraystretch}{1.2}
    \centering
    \caption{\textbf{Attribute Retrieval results on DARN dataset.} }
    % Existing works marked with stars (*) are our implementation.}
    \label{tab:DARN}
    %
    \centering 
    \scalebox{0.7}{
    \begin{tabular}{l*{10}{c}}
    \toprule
    \multirow{2}{*}{\textbf{Method}} & \multicolumn{9}{c}{\textbf{mAP for each attribute type}} & \multirow{2}{*}{\textbf{MAP}} \\
    \cmidrule(l){2-10}
     &clothes category&clothes button&clothes color&clothes length&clothes pattern&clothes shaoe&collat shaoe&sleeve length&sleeve shape \\
    \cmidrule(l){1-11}
    Random baseline                & 8.49 & 24.45 & 12.54 & 29.90 & 43.26 & 39.76 & 15.22 & 63.03 & 55.54 & 32.26 \\
    Standard triplet network       & 23.59 & 38.07 & 16.83 & 39.77 & 49.56 & 47.00 & 23.43 & 68.49 & 56.48 & 40.14 \\
    Classification network(cos)    & \textbf{43.74} & \textbf{50.82} & \textbf{52.77} & \textbf{60.83} & \textbf{59.55} & \textbf{57.06} & \textbf{44.52} & \textbf{83.53} & \textbf{66.25} & \textbf{57.54} \\
    CSN                            & 34.10 & 44.32 & 47.38 & 53.68 & 54.09 & 56.32 & 31.82 & 78.05 & 58.76 & 50.86 \\
    ASEN without ASA               & 33.94 & 45.37 & 48.56 & 54.36 & 53.83 & 57.33 & 32.78 & 77.77 & 59.32 & 51.39 \\
    ASEN without ACA               & 30.39 & 42.37 & 49.14 & 50.18 & 53.63 & 48.84 & 26.03 & 75.28 & 57.99 & 48.02 \\
    ASEN                           & \textbf{36.69} & \textbf{46.96} & \textbf{51.35} & \textbf{56.47} & \textbf{54.49} & \textbf{60.02} & \textbf{34.18} & \textbf{80.11} & \textbf{60.04} & \textbf{53.31}\\
    \bottomrule
    \end{tabular}
     }
    \end{table*}
